Bodega: Serving Linearizable Reads Locally from Anywhere at Anytime via Roster Leases

We present Bodega, the first consensus protocol that serves linearizable reads locally from any desired node, regardless of interfering writes. Bodega achieves this via a novel roster leases algorithm that safeguards the roster, a new notion of cluster metadata. The roster is a generalization of leadership; it tracks arbitrary subsets of replicas as responder nodes for local reads. A consistent agreement on the roster is established through roster leases, an all-to-all leasing mechanism that generalizes existing all-to-one leasing approaches (Leader Leases, Quorum Leases), unlocking a new point in the protocol design space. Bodega further employs optimistic holding and early accept notifications to minimize interruption from interfering writes, and incorporates smart roster coverage and lightweight heartbeats to maximize practicality. Bodega is a non-intrusive extension to classic consensus; it imposes no special requirements on writes other than a responder-covering quorum. We implement Bodega and related works in Vineyard, a protocol-generic replicated key-value store written in async Rust. We compare it to previous protocols (Leader Leases, EPaxos, PQR, and Quorum Leases) and two production coordination services (etcd and ZooKeeper). Bodega speeds up average client read requests by 5.6x-13.1x on real WAN clusters versus previous approaches under moderate write interference, delivers comparable write performance, supports fast proactive roster changes as well as fault tolerance via leases, and closely matches the performance of sequentially-consistent etcd and ZooKeeper deployments across all YCSB workloads. We will open-source Vineyard upon publication.

==> floats/fig-algo-blocks-short.tex <==
\begin{figure*}[ht!]
    \setstretch{1.05}
    \begin{minipage}{0.12\textwidth}
        \begin{mdframed}[%
                % linecolor=gray,
                linewidth=0pt,
                innertopmargin=7pt,
                innerbottommargin=7pt,
                backgroundcolor=gray!20,
                roundcorner=0pt,
                font=\small\bfseries,
                fontcolor=black!85]
            \begin{center}
                Relevant \\
                states \\
                on node $r$:
            \end{center}
        \end{mdframed}
    \end{minipage}\hspace{-5px}
    \setstretch{1.12}
    \begin{minipage}{0.872\textwidth}
        \begin{mdframed}[%
                % linecolor=gray,
                linewidth=0pt,
                leftmargin=-4pt,
                rightmargin=4pt,
                backgroundcolor=gray!8,
                roundcorner=0pt,
                font=\small,
                fontcolor=black!75]
            Normal SMR log of \avar{\color{black}\bfseries slot}s \hspace{3.2em}
            Current ballot\# \& \revise{roster}: \avar{\color{black}\bfseries bal} \ \ \avar{\color{black}\bfseries ros} \hspace{3.2em}
            Heartbeat per-peer $p$ timers: \atimer{\color{black}\bfseries heartbeat, $p$} \\
            Grantor-side timers and status sets for tracking each peer $p$ I'm granting leases to; \ Grantee-side states are similar \\
            Grantee-side per-peer $p$ local-read safety slot\#: \avar{\color{black}\bfseries thresh$_p$} \hspace{3.1em}
            Per-slot early \texttt{AcceptNote} markers: \aset{\color{black}\bfseries accnote, \avar{\color{black}\bfseries slot}}
        \end{mdframed}
    \end{minipage}%

    \vspace*{5pt}
    \setstretch{1.0}
    
    \begin{minipage}[t]{0.39\textwidth}
        \begin{algoblock}[%
            frametitle={Proactive \revise{roster} change to \avpm{ros}:},
            frametitlebackgroundcolor=\acviolet]
            \begin{algolistnonum}
                \item get new roster \avpm{ros} from user or according to stats, and do \afun{announce\_\revise{roster}}{\avar{bal}, \avpm{ros}}
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-8pt}
            \begin{tikzpicture}[y=0.2cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[-, line width=1.5pt, draw=Orchid!75] (A) -- (B);
            \end{tikzpicture}
            \hspace{35pt}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Upon \atimer{heartbeat, $p$} timeout for peer $p$:},
            frametitlebackgroundcolor=\acviolet]
            \begin{algolistnonum}
                \item create new roster \avpm{ros} with $p$'s special roles removed, and do \afun{announce\_\revise{roster}}{\avar{bal}, \avpm{ros}}
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-5pt}
            \begin{tikzpicture}[y=0.3cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=Orchid!75] (A) -- (B);
            \end{tikzpicture}
            \hspace{23pt}
            \begin{tikzpicture}[y=0.3cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=Orchid!75] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Do\,\,\,\afun{announce\_\revise{roster}}{\avar{bal}, \avpm{ros}}:},
            frametitlebackgroundcolor=\acviolet]
            \begin{algolistnonum}
                \item compose a unique higher ballot\# \avpm{bal}, broadcast \amsg{Heartbeat}{\avpm{bal}, \avpm{ros}} to all
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-5pt}
            \begin{tikzpicture}[y=0.3cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=Orchid!75] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}

        \begin{algoblock}[%
            frametitle={Recv \amsg{Heartbeat}{\avpm{bal}, \avpm{ros}} $\leftarrow$ $p$:},
            frametitlebackgroundcolor=\acorange]
            \begin{algolistnonum}
                \item if \avpm{bal} $>$ current ballot \avar{bal}:
                    \begin{algolistnonum}
                        \item do \afun{revoke\_leases}{\avar{bal}}, set \avpm{bal} and \avpm{ros}, then do \afun{initiate\_leases}{\avpm{bal}};
                        \item if I'm leader of \avpm{ros}: re-\texttt{Prepare} in-progress slots
                    \end{algolistnonum}
                \vspace{6pt}
                \hrule
                \vspace{2pt}
                \item refresh heartbeat timer \atimer{heartbeat, $p$}
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-5pt}
            \begin{tikzpicture}[y=0.3cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=YellowOrange!80] (B) -- (A);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Repeat every heartbeat interval:},
            frametitlebackgroundcolor=\acorange]
            \begin{algolistnonum}
                \item broadcast \amsg{Heartbeat}{\avar{bal}, \avar{ros}} to all;
                \item for each $p$ I'm endowing: extend timer by \atmdur{lease}$+$\atmdur{$\Delta$}, and piggyback lease \amsg{Renew}{\avar{bal}};
                \item for each endowing $p$: piggyback \amsg{RenewReply}{\avar{bal}}
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-5pt}
            \begin{tikzpicture}[y=0.3cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=YellowOrange!80] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Recv lease \amsg{Renew}{\avar{bal}} $\leftarrow$ $p$:},
            frametitlebackgroundcolor=\acorange]
            \begin{algolistnonum}
                \item if $p$ in endowed set: kickoff \atimer{endowed, $p$} by \atmdur{lease}$-$\atmdur{$\Delta$}
            \end{algolistnonum}
        \end{algoblock}

            \begin{center}
            \vspace{-5pt}
            \begin{tikzpicture}[y=0.3cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=YellowOrange!80] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Recv \amsg{RenewReply}{\avar{bal}} $\leftarrow$ $p$:},
            frametitlebackgroundcolor=\acorange]
            \begin{algolistnonum}
                \item if $p$ in endowing set: kickoff \atimer{endowing, $p$} by \atmdur{lease}$+$\atmdur{$\Delta$}
            \end{algolistnonum}
        \end{algoblock}
    \end{minipage}%
    \begin{minipage}[t]{0.03\textwidth}
        \begin{center}
            \begin{tikzpicture}[x=0.27cm,y=0.35cm,baseline=(current bounding box.north)]
                \path[use as bounding box] (0,0) -- (2,-33);
                \coordinate (A) at (0,   -17.22);
                \coordinate (B) at (0.9, -17.22);
                \coordinate (C) at (0.8, -17.22);
                \coordinate (D) at (0.8, -0.9);
                \coordinate (E) at (0.7, -0.9);
                \coordinate (F) at (2,   -0.9);
                \coordinate (G) at (2,   -32.5);
                \coordinate (H) at (1.1, -32.5);
                \coordinate (I) at (1.2, -32.5);
                \coordinate (J) at (1.2, -19.3);
                \coordinate (K) at (1.3, -19.3);
                \coordinate (L) at (0,   -19.3);
                \draw[-,  line width=1.5pt, draw=Maroon!70] (A) -- (B);
                \draw[-,  line width=1.5pt, draw=Maroon!70] (C) -- (D);
                \draw[->, line width=1.5pt, draw=Maroon!70] (E) -- (F);
                \draw[-,  line width=1.5pt, draw=Maroon!70] (G) -- (H);
                \draw[-,  line width=1.5pt, draw=Maroon!70] (I) -- (J);
                \draw[->, line width=1.5pt, draw=Maroon!70] (K) -- (L);
            \end{tikzpicture}
        \end{center}
    \end{minipage}%
    \begin{minipage}[t]{0.26\textwidth}
        \begin{algoblock}[%
            frametitle={Do\,\,\,\afun{revoke\_leases}{\avar{bal}}:},
            frametitlebackgroundcolor=\acred]
            \begin{algolistnonum}
                \item broadcast lease \amsg{Revoke}{\avar{bal}};
                \item for every $p$ I was endowing, wait until: either \amsg{RevokeReply}{\avar{bal}} is received from $p$, or $p$ gets removed from the set by timeout
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-4.5pt}
            \begin{tikzpicture}[y=0.35cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=Maroon!70] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Recv \amsg{Revoke}{\avar{bal}} $\leftarrow$ $p$:},
            frametitlebackgroundcolor=\acred]
            \begin{algolistnonum}
                \item if \avar{bal} $\geqslant$ current ballot: remove $p$ from grantee-side sets;
                \item send \amsg{RevokeReply}{\avar{bal}} back
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-4.5pt}
            \begin{tikzpicture}[y=0.35cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=Maroon!70] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Do\,\,\,\afun{initiate\_leases}{\avar{bal}}:},
            frametitlebackgroundcolor=\acred]
            \begin{algolistnonum}
                \item start lease guard phase, broadcast \amsg{Guard}{\avar{bal}, \avar{thresh}} to all, where \avar{thresh} is the highest slot\# I have ever accepted;
                \item for every peer $p$:
                    \begin{algolistnonum}
                        \item wait until \amsg{GuardReply}{\avar{bal}} is received, or retry if timeout;
                        \item start endowing $p$, kickoff timer
                    \end{algolistnonum}
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-4.5pt}
            \begin{tikzpicture}[y=0.35cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=Maroon!70] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Recv \amsg{Guard}{\avar{bal}, \avar{thresh}} $\leftarrow$ $p$:},
            frametitlebackgroundcolor=\acred]
            \begin{algolistnonum}
                \item if \avar{bal} $\ne$ current ballot: ignore;
                \item if $p \notin$ grantee-side sets: record \avar{thresh}$_p$ for later local read checks, kickoff guard timer, and send \amsg{GuardReply}{\avar{bal}} back
            \end{algolistnonum}
        \end{algoblock}

        \vspace{12pt}

        \begin{algoblock}[%
            frametitle={Upon lease timer \atimer{{\color{darkgray!75}\normalfont \_}, $p$} timeout:},
            frametitlebackgroundcolor=\acgold]
            \begin{algolistnonum}
                \item remove $p$ from corresponding set
            \end{algolistnonum}
        \end{algoblock}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.30\textwidth}
        \begin{algoblock}[%
            frametitle={Handle \amsg{Write}{$k$, $v$} req $\leftarrow$ client:},
            frametitlebackgroundcolor=\acblue]
            \begin{algolistnonum}
                \item if I'm leader: \texttt{Accept} phase at next \avar{slot} just like normal consensus, except:
                    \begin{algolistnonum}
                        \item leader decides commit only after all responders of $k$ in \avar{ros} have replied;
                        \item all nodes broadcast \amsg{AcceptNote}{\avar{bal}, \avar{slot}} to responders of $k$, besides replying \amsg{AcceptReply}{\avar{bal}, \avar{slot}} to leader
                    \end{algolistnonum}
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-5pt}
            \begin{tikzpicture}[y=0.3cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=RoyalBlue!50] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Recv \amsg{AcceptNote}{\avar{bal}, \avar{slot}} $\leftarrow$ $p$:},
            frametitlebackgroundcolor=\acblue]
            \begin{algolistnonum}
                \item if \avar{bal} $=$ current ballot prepared at \avar{slot}: add $p$ to \aset{accnote, \avar{slot}}
            \end{algolistnonum}
        \end{algoblock}
        
        \vspace{9pt}
        
        \begin{algoblock}[%
            frametitle={Handle \amsg{Read}{$k$} req $\leftarrow$ client:},
            frametitlebackgroundcolor=\acgreen]
            \begin{algolistnonum}
                \item if $|$\aset{endowed}$|$ $< m$, or if I'm not a responder of $k$ in current \revise{roster} \avar{ros}, or if there's no size-$m$ subset of \aset{endowed} where I have committed all slots up to \avar{thresh}$_p$ for all $p$ in the subset:
                    \begin{algolistnonum}
                        \item treat as normal consensus cmd;
                    \end{algolistnonum}
                \item else if I'm the {\color{black!50} (stable)} leader of \avar{ros}:
                    \begin{algolistnonum}
                        \item reply with latest committed val of $k$;
                    \end{algolistnonum}
                \item else{\color{black!50}, (I'm a non-leader responder in \avar{ros})}:
                    \begin{algolistnonum}
                        \item do \afun{responder\_read}{$k$}
                    \end{algolistnonum}
            \end{algolistnonum}
        \end{algoblock}

        \begin{center}
            \vspace{-5pt}
            \begin{tikzpicture}[y=0.3cm]
                \coordinate (A) at (0, 0);
                \coordinate (B) at (0, -1);
                \draw[->, line width=1.5pt, draw=ForestGreen!60] (A) -- (B);
            \end{tikzpicture}
            \vspace{-3pt}
        \end{center}
        
        \begin{algoblock}[%
            frametitle={Do\,\,\,\afun{responder\_read}{$k$}:},
            frametitlebackgroundcolor=\acgreen]
            \begin{algolistnonum}
                \item find highest \avar{slot}$_k$ containing write to $k$;
                \item if \avar{slot}$_k$ has committed, or is accepted at current \avar{bal} and $|$\aset{accnote, \avar{slot}$_k$}$|$ $\geqslant m$:
                    \begin{algolistnonum}
                        \item reply with the value in \avar{slot}$_k$;
                    \end{algolistnonum}
                \item else: hold until the above becomes true, promptly redirect after \atmdur{unhold} timeout
            \end{algolistnonum}
        \end{algoblock}
    \end{minipage}
    
    \captionsetup{justification=raggedright}
    \vspace{-6pt}
    \floatcapoffig{\revise{High-level Summary of \bodega}}{Lists the actions a node $r$ would take, grouped by purposes for clarity: \acbox{\acviolet} triggers for a new \revise{roster}, \acbox{\acred} granting new \revise{roster} leases, \acbox{\acorange} heartbeats and lease renewals, \acbox{\acblue} handling client writes, \acbox{\acgreen} handling client reads. \revise{Arrows annotate a natural reading order that follows the usual flow of the protocol. See appendix Figure~\ref{fig:algo-blocks-full} for the full version.}}
    \label{fig:algo-blocks}
\end{figure*}


==> sections/3-design-andrea.tex <==
\section{Design}
\label{sec:design}


In this section, we present the core design of \bodega, an always-local linearizable read protocol.

\paratitle{Design Outline}
We derive the complete design in three steps: \circleb{1} define \revise{the roster}, \circleb{2} design optimal normal case operations assuming replicas agree on the same stable \revise{roster}, and \circleb{3} introduce background \revise{roster} leases, the enabler behind the fault-resilient agreement on the \revise{roster}.

For clarity, we adhere to Paxos-style terminology throughout this paper. All the optimizations are applicable to Raft-style protocols due to their fundamental duality~\cite{parallel-paxos-raft}.


\subsection{\revise{The Roster}}
\label{sec:design-roster}

\revise{We start by introducing the core concepts behind \bodega: responder status and the roster.} A node is a \textit{responder} for a key if it is expected to serve read-only requests on that key locally without actively contacting other nodes. A \textit{\revise{roster}} is the collection of each node's desired capabilities at a certain time. Specifically, it dictates:

\begin{itemize}
    \item The node ID of the current leader node.
    \item For each (range of) key(s): the node IDs of its responders.
\end{itemize}

\noindent The \revise{roster} is a generalization of leadership from classic protocols: besides the one special leader role, we now have special responder roles for selected keys. The leader can be implicitly treated as a responder for all keys, \revise{and different keys can additionally mark different nodes as responders.}

\revise{The optimal choice of responders for each key depends on various factors: \circleb{1} client locations and proximity, \circleb{2} workload read-heaviness and skewness on the key, and \circleb{3} cluster topology and status (e.g., if a node is exceptionally distant or lagging). This paper focuses on the mechanisms supporting the roster rather than the policies for tuning it; we recognize that the latter could be an intriguing study on its own.}

The system starts from an empty \revise{roster} with a null leader ID and an empty responder set for the entire keyspace. Every newly-proposed \revise{roster} is associated with (and identified by) a unique ballot number, forming a $\langle$\avar{bal}, \avar{ros}$\rangle$ pair, where \avar{bal} is the ballot number formed by concatenating a monotonically increasing integer $b$ with the proposing node's ID $r$ to ensure uniqueness. \revise{Rosters} of different ballots may contain the same content but are still considered different. \revise{Roster changes may happen due to explicit requests by users, automatic tuning from statistics, or mandatorily in reaction to failures.}


\subsection{Normal Case Operations}
\label{sec:design-normal-case}

We first describe normal case operations, using Figure~\ref{fig:design-agreed-roster} as a demonstrative example. In a 5-node cluster, S0 is the leader (depicted by the crown) and S2,3,4 are additional responders (depicted by the red star symbols) for a \revise{specific} key $k$. Assume, in this section, that this is the latest \revise{roster} all nodes know and consider stable according to leases. \revise{Nodes use this common roster to assure that writes to $k$ would never commit before reaching all of its active responders. A responder can therefore serve reads directly if it knows the latest value of $k$ will commit; when unsure, it optimistically holds the read locally until that decision becomes certain.}

% Given the definition of rosters, the rest of the design can be decoupled into two parts: normal case operations under an agreed roster and reaching agreement on the roster.

\subsubsection{Writes}
\label{sec:design-normal-case-writes}

Writes follow the same leader-based process as in MultiPaxos \revise{(Figure~\ref{fig:design-agreed-roster} blue arrows)}, except for an updated commit condition. Normally, a write to key $k$ can be marked as committed and acknowledged once $\geqslant m$ \texttt{AcceptReply}s are received. We impose an additional constraint that it must also have received replies from all the responders for $k$, according to the leader's current \revise{roster}.

Requiring a write quorum that covers all responders is an unavoidable penalty that any local linearizable read algorithm must pay. Luckily, without far-off responders, this penalty is marginal as the system usually picks a leader with relatively uniform distances to other replicas, and the write must anyway reach a majority. This aligns with previous observations~\cite{quorum-leases} and our evaluation results (\S\ref{sec:evaluation}). Distant responders could still be appropriate for certain workloads.


\input{floats/fig-design-agreed-roster}


\subsubsection{Reads}
\label{sec:design-normal-case-reads}

Clients send read-only requests on key $k$ to the closest responder server for $k$ \revise{(Figure 4 green arrows)}. It is common for clients of wide-area systems to be co-located with some replica; for example, consensus is usually part of an outer system, e.g., a database, where requests come directly from participating sites, but this is not a requirement.

% Servers that expect read-heavy workloads from nearby clients should be marked as responders for corresponding keys.

When a server S (with a stable \revise{roster}) takes a read, there are three cases. \circleb{1} S is the leader, in which case S simply finds the highest committed slot in its log that contains a write to $k$ and returns the value; if none are found, it returns null. The leader does not need to worry about in-progress writes~\cite{paxos-made-live}. \circleb{2} S is neither a leader nor a responder for $k$ (e.g., S1 in Fig.~\ref{fig:design-agreed-roster}), in which case S  rejects the read and redirects the client to another server, preferably a nearby responder or the leader. \circleb{3} S is a non-leader responder. In this case, S looks up the highest slot in its log that contains any write to $k$.  If the slot is in committed status, S immediately replies with the value (e.g., the read at S4 in Fig.~\ref{fig:design-agreed-roster}); otherwise, S cannot yet determine whether that value will commit or may be overwritten due to an impending failure (e.g., the read at S3), in which case, S optimistically  \textit{holds} the read.

% ; this is when a follower local read takes action

\paratitle{Optimistic Holding}
The holding mechanism is optimistic in that it expects S and its connection with the leader to remain healthy and for the slot to be committed soon.  In failure-free cases, S may need to wait up to one RTT to be notified that an interfering write has committed (from when S receives the \texttt{Accept} from leader and replies to it, to when S receives the \texttt{Commit} notification). Note that even with a constant stream of writes, held reads will not be blocked indefinitely: they are released as soon as their associated slot turns committed.

\if 0
from the perspective of an interfering write, a local read could arrive at S at any time during a 2-message-delay window: from when S receives the \texttt{Accept} from leader (and replies to it) to when S gets the \texttt{Commit} notification. Therefore, a pending read could be released as soon as instantly or as late as one RTT to the leader. 
\fi 

A responder S optimistically holds a local read by adding it to a \textit{pending set} attached to the corresponding slot. Upon receiving the commit notification for a slot, S releases the pending reads and replies with the committed value.  To handle cases where the leader does not respond to S within one RTT, clients start an \textit{unhold} timeout when sending local read requests; if the timeout is reached, clients proactively issue the same request to another responder or the leader (with the same req ID, which is safe since reads are idempotent) and use the earliest reply. A good timeout length is longer than the usual RTT between S and the current leader.

\paratitle{Early Accept Notifications}
While optimistic holding already delivers outstanding local read performance, \bodega\ introduces a further optimization \revise{that reduces average holding time}: followers reply to \texttt{Accept}s on key $k$ not only to the leader, but also broadcast \texttt{AcceptNote} notifications to $k$'s responders. Once a responder S has received $m$ \texttt{AcceptNote}s (counting self), it can then assert that a pending slot will commit, even across minority failures.  A similar optimization exists for BFT writes~\cite{pbft-recovery}.  On average, this optimization halves the expected holding time for interfered local read in \bodega.

\if 0
applies it to local reads and allows selective notifications to only $k$'s responders.
\fi


\subsection{\revise{Roster} Leases}
\label{sec:design-roster-leases}

So far, we have assumed a consistent \revise{roster} agreed across the cluster without showing how it is achieved.  The basic idea is to establish a roster lease, an $m$-to-$r$ lease, between a majority of nodes in the cluster and all nodes that may be responders for some key.  With this roster lease, responders know that the roster is stable: thus the leader also knows the identity of all responders and will not perform writes without notifying these responders. 

\if 0
At first glance, this problem might seem solvable by encoding \revise{roster} changes as special consensus commands and using normal consensus to establish agreement. However, this approach is not fault-tolerant and would easily lead to system-wide hang when a responder fails. This is because on-the-fly writes are required to wait for replies from all responders to ensure the safety of potential local reads, which blocks execution and prevents later \revise{roster} changes from taking effect.
\fi

We present how \bodega deploys off-the-critical-path \textit{roster leases} to establish a stable \revise{roster} elegantly and efficiently. We use Figure~\ref{fig:design-roster-leases} as an llustration when needed. 

\paratitle{Lease-related States}

The intuition behind \revise{roster} leases is to let all replicas act as both a lease grantor and a grantee, exchanging lease grants in an \textit{all-to-all} pattern to protect the highest-ballot \revise{roster} seen. Recall \S\ref{sec:bg-distributed-leases} for how a standard lease grant works.

Besides the SMR log and the $\langle$\avar{bal}, \avar{ros}$\rangle$ pair, we let every node S \revise{play both the roles of a lease grantor and a grantee, effectively creating an all-to-all lease granting pattern}. This means S maintains the following additional data structures: \circleb{1} two lists of grantor-side timers \atimer{guarding, $p$} and \atimer{endowing, $p$}, one each per peer node P; \circleb{2} two corresponding sets \aset{guarding} and \aset{endowing} for tracking which peers are S currently guarding/endowing to; \circleb{3} two lists of grantee-side timers \atimer{guarded, $p$} and \atimer{endowed, $p$}, one each per peer P; \circleb{4} two corresponding sets \aset{guarded} and \aset{endowed} for tracking the guards/endowments S currently holds; \circleb{5} a list of safety slot numbers \avar{thresh$_p$}, whose usage will become clear soon.

\subsubsection{\revise{Roster} Leases Activation}
\label{sec:design-roster-leases-activation}

We first describe how \revise{roster} leases are activated. Consider node S wants to announce a new \revise{roster} \avpm{ros}; this could be due to, e.g., stepping up as new leader (by setting S as the leader in \avpm{ros}) or other reasons covered in \S\ref{sec:design-roster-leases-expiration}. S composes a unique, higher ballot \avpm{bal} by concatenating $(b+1)$ with its node ID, where $b$ is the higher part of the current \avar{bal}. S then broadcasts the $\langle$\avpm{bal}, \avpm{ros}$\rangle$ pair to all nodes including self.

For any node S upon receiving a ballot \avpm{bal} higher than ever seen, it first ensures all old leases are safely revoked (covered in \S\ref{sec:design-roster-leases-expiration}). Then, it moves on to $\langle$\avpm{bal}, \avpm{ros}$\rangle$ and begins the \afun{initiate\_leases}{\avpm{bal}} procedure, where it starts granting leases to all peers asynchronously in parallel.

% invalidated
% updates the pair to

To each peer P, the procedure obeys standard lease granting: S and P first exchange a round of \texttt{Guard} and \texttt{GuardReply}, kicking off their \atimer{guarding} or \atimer{guarded} timer by \atmdur{guard}$\pm$\atmdur{$\Delta$} and adding the other side to their \aset{guarding} or \aset{guarded} set, respectively. If S receives P's \texttt{GuardReply} before its \atimer{guarding} timeout, the guard succeeds so S moves P to \aset{endowing} and sends \texttt{Renew} to P; otherwise, S retries the guard. On P, if it receives a \texttt{Renew} before \atimer{guarded} timeout, it moves S to \aset{endowed}, replies with \texttt{RenewReply}, kicks off \atimer{endowed} by \atmdur{lease}$-$\atmdur{$\Delta$}, and starts expecting periodic \texttt{Renew}s from S. If the first \texttt{RenewReply} fails to reach S, S waits for a safe \atmdur{guard}$+$\atmdur{lease}$+$\atmdur{$\Delta$} before retrying the guard~\cite{quorum-leases}. Otherwise, S repeats \texttt{Renew} for at least once every \atmdur{lease} to keep the lease refreshed. On any server S, whenever a \atimer{intent, $p$} times out for any intent among the four, P is removed from the corresponding set \aset{intent}.

Finally, after transitioning to \avpm{ros}, if S sees itself being the leader of \avpm{ros}, it does the usual step-up routine of redoing the \texttt{Prepare} phase for non-committed slots of its log.

% conducts


\paratitle{Stable Condition \& Safety Thresholds}
As shown in \S\ref{sec:bg-distributed-leases} and above, a node P is considered granted a lease by S when S $\in$ P's \aset{endowed} set. Assume P itself is always in the set. The size of this set, $|$\aset{endowed}$|$, indicates the number of lease grants P currently holds. When $|$\aset{endowed}$|$ $\geqslant m$, then P knows that at least a majority number of nodes in the cluster has the same latest $\langle$\avar{bal}, \avar{ros}$\rangle$ as P and that only one such \revise{roster} exists; this is called the \textit{stable} \revise{roster} of the cluster and is a necessary precondition for all optimizations described in \S\ref{sec:design-normal-case}. For example, in Figure~\ref{fig:design-roster-leases}, the local reads at S1 and S2 are rejected due to an insufficient lease count.

However, this condition alone is not enough. When a node directly inspects its log and uses the highest slot index for local reads, it is assuming that its log is up-to-date and contains all the recently accepted instances; this is normally true but could be violated when a fell-behind node joins a new \revise{roster}. To address this, we let \texttt{Guard} messages from S to P carry an extra number, which is the highest slot number that S has ever accepted. P stores the number in its \avar{thresh} list. A node permits local reads only if it has committed all the slots up to the $m$-th smallest slot number in its \avar{thresh} list. S4 in Figure~\ref{fig:design-roster-leases}, for example, has not reached this condition.

In summary, all the stable leader and local read operations of \S\ref{sec:design-normal-case} are preceded by the following stable condition check:
\begin{align} \label{eqn:stable-condition}
    & |\text{\{\}}_{\text{endowed}}| \geqslant m \\
    & \wedge \,\, \exists \text{ size-}m \text{ subset } E \subseteq \text{\{\}}_{\text{endowed}}: \nonumber \\[-2pt]
    & \quad\,\,\,\,\,\,\, \text{ committed all slots up to \textit{thresh}}_p, \forall p \in E \nonumber
\end{align}
\noindent If the check fails, the operation falls back to classic consensus as if it is a write, which does not require this check.


\input{floats/fig-design-roster-leases}

\input{floats/fig-timeline-comparison}


\subsubsection{Revocation \& Expiration}
\label{sec:design-roster-leases-expiration}

Most \revise{roster} lease activations happen when there are ongoing old leases in the system. Broadly speaking, a \revise{roster} change may be triggered by one of the following reasons.

\begin{itemize}
    \item Node initiates a new \revise{roster} in reaction to suspected failures, removing failed nodes from special responder roles.
    \item Node autonomously proposes a new, more optimized \revise{roster} according to collected workload statistics.
    \item Node receives an explicit \revise{roster} change request from user.
\end{itemize}

\noindent In either case, before \afun{initiate\_leases}{}, a node S always invokes the \afun{revoke\_leases}{\avar{bal}} procedure synchronously to ensure that all the leases it is granting or holding with the older ballot \avar{bal} are safely revoked and removed. To do so, S clears its \aset{guarding} set and broadcasts \texttt{Revoke} messages carrying the old ballot. Whenever a node P receives a \texttt{Revoke} with matching ballot from S, it removes S from the \aset{guarded} and \aset{endowed} sets and replies with \texttt{RevokeReply}.

S either receives a \texttt{RevokeReply} from P promptly (common fast case) or has to wait for expiration timeout (failure case), after which it removes P from \aset{endowing}. \revise{Note that, unless failures occur and force a wait on expiration, a roster change completes swiftly within two message rounds: one for the revocation and the other for the initiation guards.}

\subsubsection{Piggybacking on Heartbeats}
\label{sec:design-roster-leases-piggyback}

Heartbeats are ubiquitous in modern distributed systems; many systems already deploy all-to-all heartbeats for tasks such as health tracking~\cite{etcd, zookeeper, epaxos, rabbitmq}. This opens the opportunity to enable \revise{roster} leases without any common-case overheads, by piggybacking lease messages onto existing periodic heartbeats. \bodega piggybacks all the \texttt{Renew} and \texttt{RenewReply} messages onto heartbeats, and uses a proper heartbeat interval \atmdur{hb\_send} such that leases are refreshed in time. Heartbeat messages also carry the sender's $\langle$\avar{bal}, \avar{ros}$\rangle$ pair to let receivers discover \revise{roster} changes.

Each node has per-peer timers \atimer{heartbeat, $p$} which are used for detecting failures from peers; a peer is considered down if no heartbeats were received from it for \atmdur{hb\_fail}. A rule of thumb for choosing good timeout lengths for a cluster is:
\begin{align}
    \text{avg. RTT} < \text{\atmdur{hb\_send}} \ll \text{\atmdur{hb\_fail}} < \text{\atmdur{guard}} = \text{\atmdur{lease}}
\end{align}
\noindent \bodega uses the following defaults for wide-area replication: \atmdur{hb\_send} $=$ 120ms, \atmdur{hb\_fail} $\approx$ 1200ms, \atmdur{guard} $=$ \atmdur{lease} $=$ 2500ms.


% \input{floats/fig-algo-blocks}
% \input{floats/fig-algo-blocks-separate}  % using png fig to make format checker happy for now...


\subsection{\revise{Summary of \bodega}}
\label{sec:design-summary-algo}

% \revise{Figure~\ref{fig:algo-blocks} shows a high-level summary of the \bodega protocol.}

\revise{We provide a complete presentation of the \bodega protocol in Figure~\ref{fig:algo-blocks-full} of Appendix~\ref{sec:appendix-full-algo} as an implementation guide.}

